How Out-of-Distribution Detection Learning Theory Enhances Transformer: Learnability and Reliability

Transformers excel in natural language processing and computer vision tasks. However, they still face challenges in generalizing to Out-of-Distribution (OOD) datasets, i.e. data whose distribution differs from that seen during training. OOD detection aims to distinguish outliers while preserving in-distribution (ID) data performance. This paper introduces the OOD detection Probably Approximately Correct (PAC) Theory for transformers, which establishes the conditions for data distribution and model configurations for the OOD detection learnability of transformers. It shows that outliers can be accurately represented and distinguished with sufficient data under conditions. The theoretical implications highlight the trade-off between theoretical principles and practical training paradigms. By examining this trade-off, we naturally derived the rationale for leveraging auxiliary outliers to enhance OOD detection. Our theory suggests that by penalizing the misclassification of outliers within the loss function and strategically generating soft synthetic outliers, one can robustly bolster the reliability of transformer networks. This approach yields a novel algorithm that ensures learnability and refines the decision boundaries between inliers and outliers. In practice, the algorithm consistently achieves state-of-the-art (SOTA) performance across various data formats.

==> content/6_experiment.tex <==
\section{Experiments}\label{Experiments}
\label{sec:exp}

In this section, we provide empirical evidence to validate the effectiveness of \textsc{GROD} across a range of real-world classification tasks and types of outliers. We conduct extensive comparison experiments using four transformer backbones on various NLP and CV tasks. Additionally, we perform an ablation study to analyze the impact of key parameters and modules within \textsc{GROD}.

\paragraph{Settings.}
\begin{table}[!ht]
    \centering % 使内容在 wrapfigure 分配的宽度内居中
    \caption{Image and text datasets for experiments.} % 表格标题
    \label{datasets} % 建议为环绕表格使用新的标签
    \resizebox{\linewidth}{!}{ % 将表格缩放到 wrapfigure 环境的宽度
        \begin{tabular}{ccccc}
        \toprule
            \multicolumn{5}{c}{Image Datasets}\\ \midrule
            \multicolumn{2}{c}{ID} & \multicolumn{2}{c}{Near-OOD} & Far-OOD \\ \cmidrule(r){1-2}\cmidrule(r){3-4}\cmidrule(r){5-5}
            \multirow{2}{*}{Classical} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{Tiny ImageNet} & \multirow{3}{*}{\textbf{SVHN}} \\ 
            ~ & \textbf{CIFAR-100} & \textbf{CIFAR-10} & \textbf{Tiny ImageNet} & ~ \\ 
            Large-scale & \textbf{ImageNet-200} & \textbf{CIFAR-10} & \textbf{CIFAR-100 }& ~ \\ \toprule
            \multicolumn{5}{c}{Text Datasets} \\ \midrule
            ~ & \multicolumn{2}{c}{ID} & \multicolumn{2}{c}{OOD} \\ 
            \cmidrule(r){2-3}\cmidrule(r){4-5}
            Semantic Shift & \multicolumn{2}{c}{\textbf{CLINC150} with intents} & \multicolumn{2}{c}{\textbf{CLINC150} without intents}  \\ 
            Background Shift & \multicolumn{2}{c}{\textbf{IMDB}} & \multicolumn{2}{c}{\textbf{Yelp}} \\ \bottomrule
        \end{tabular}
    }
    % \vspace{-\intextsep} % 可选：减少表格下方的一些垂直间距
\end{table}

We use \textsc{GROD} to strengthen the reliability of pre-trained backbone models: ViT-B-16 \citep{dosovitskiy2020image} for CV tasks, and encoder-only BERT \citep{devlin2018bert} and decoder-only GPT-2 small \citep{radford2019language} and Llama-3.1-8B for NLP tasks. Datasets are summarized in Table \ref{datasets}.
We assess model performance using ID classification accuracy (ID ACC) and binary classification metrics for ID vs. OOD: FPR@95 (F), AUROC {A}, AUPR\_IN (I), and AUPR\_OUT (O). The diverse experimental setup comprehensively evaluates the performance of \textsc{GROD}, and detailed settings, models and dataset information are in Appendix~\ref{appendix settings}.

\paragraph{Main results.}



Several prevalent methods are used for comparison, \textit{i.e.} \textsc{MSP} \citep{hendrycks2016baseline}, \textsc{ODIN} \citep{liang2017enhancing}, \textsc{VIM} \citep{wang2022vim}, \textsc{GEN} \citep{liu2023gen}, and \textsc{ASH} \citep{djurisic2022extremely} which require only post-processing, and finetuning models \textsc{G-ODIN} \citep{hsu2020generalized}, \textsc{NPOS} \citep{tao2023non}, \textsc{CIDER} \citep{ming2022exploit}, \textsc{OE} \citep{hendrycks2018deep}, \textsc{\textsc{MIXOE}} \citep{zhang2023mixture}, \textsc{ATOM} \citep{chen2021atom}, \textsc{POEM} \citep{ming2022poem}, and \textsc{DivOE} \citep{zhu2023diversified}. All the baselines are offered in or adapted into the OpenOOD benchmark \citep{zhang2023openood,yang2022openood,yang2022fsood,yang2021generalized,bitterwolf2023or}. 
% \begin{table}
%     \centering
%     \caption{Image and text datasets for experiments.}
%     \label{datasets}
%     \resizebox{0.5\textwidth}{!}{
%     \begin{tabular}{ccccc}
%     \toprule
%         \multicolumn{5}{c}{Image Datasets}\\ \midrule
%         \multicolumn{2}{c}{ID} & \multicolumn{2}{c}{Near-OOD} & Far-OOD \\ \cmidrule(r){1-2}\cmidrule(r){3-4}\cmidrule(r){5-5}
%         \multirow{2}{*}{Classical} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{Tiny ImageNet} & \multirow{3}{*}{\textbf{SVHN}} \\ 
%         ~ & \textbf{CIFAR-100} & \textbf{CIFAR-10} & \textbf{Tiny ImageNet} & ~ \\ 
%         Large-scale & \textbf{ImageNet-200} & \textbf{CIFAR-10} & \textbf{CIFAR-100 }& ~ \\ \toprule
%         \multicolumn{5}{c}{Text Datasets} \\ \midrule
%         ~ & \multicolumn{2}{c}{ID} & \multicolumn{2}{c}{OOD} \\ 
%         \cmidrule(r){2-3}\cmidrule(r){4-5}
%         Semantic Shift & \multicolumn{2}{c}{\textbf{CLINC150} with intents} & \multicolumn{2}{c}{\textbf{CLINC150} without intents}  \\ 
%         Background Shift & \multicolumn{2}{c}{\textbf{IMDB}} & \multicolumn{2}{c}{\textbf{Yelp}} \\ \bottomrule
%     \end{tabular}
%     }
% \end{table}

\begin{table*}[!ht]
    \centering
    % \small
    \caption{Quantitative comparison of CV tasks with prevalent methods of the ID classification and OOD detection performance on \textbf{ViT backbone}. \textbf{The average performance of three OOD datasets} is reported.  The red, blue and bold fonts denote Top 1,2,3 in ranking.}
    \label{CV experiments}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccccccccccccc}
    \toprule
        \multicolumn{2}{c}{ID Datasets}  &\multicolumn{5}{c}{\textbf{CIFAR-10}}  &\multicolumn{5}{c}{\textbf{CIFAR-100}} &\multicolumn{5}{c}{\textbf{ImageNet-200}}  \\ \cmidrule(r){1-2}\cmidrule(r){3-7}\cmidrule(r){8-12}\cmidrule(r){13-17}

        \multicolumn{2}{c}{Evaluate Metrics (\%)}  &ID ACC$\uparrow$  &F $\downarrow$ &A $\uparrow$ &I$\uparrow$ &O$\uparrow$ &ID ACC$\uparrow$  &F $\downarrow$ &A $\uparrow$ &I$\uparrow$ &O$\uparrow$ &ID ACC$\uparrow$  &F $\downarrow$ &A $\uparrow$ &I$\uparrow$ &O$\uparrow$ \\ 
        \cmidrule(r){1-2}\cmidrule(r){3-7}\cmidrule(r){8-12}\cmidrule(r){13-17}
        
        Baseline & \textsc{MSP} & 96.16 &21.97 &93.62 &93.65 &93.29 & 84.34 & 57.34  & 81.13  & 77.78  & 82.54  &89.09 &19.46 &\textcolor{blue}{95.18} &\textbf{95.26} &\textcolor{blue}{94.84} \\ \cdashline{1-2}\cdashline{3-7}\cdashline{8-12}\cdashline{13-17}
        
        
        \multirow{4}{*}{PostProcess} & \textsc{ODIN}  &\multirow{4}{*}{96.16} &26.35 &94.35 &92.99 &95.38 & \multirow{4}{*}{84.34}  & 63.29  & 80.30  & 74.81  & 83.97 &\multirow{4}{*}{89.09} &32.67 &92.23 &92.70 &92.64  \\
        
        ~ & \textsc{VIM}  & ~&11.12 &\textbf{97.74} &\textbf{97.64} &97.77 & ~  & 36.07  & 90.55  & \textcolor{blue}{89.33}  & 90.43  &~ &23.92 &92.96 &92.97 &91.76 \\ 
        
        ~ & \textsc{GEN}  & ~&18.46 &95.85 &95.41 &96.07 & ~  & 51.53  & 86.97  & 83.56  & 87.77 &~ &29.68 &85.35 &87.98 &79.99  \\ 
        
        ~ & \textsc{ASH}  & ~&17.71 &96.08 &95.75 &96.20 & ~ & 51.94  & 86.82  & 83.38  & 87.64  & ~&24.88 &94.53 &93.76 &94.05 \\ \cdashline{1-2}\cdashline{3-7}\cdashline{8-12}\cdashline{13-17}
        
        \multirow{6}{*}{\makecell{Finetuning+ \\ PostProcess}} & \textsc{G-ODIN}  &95.56 &70.00 &81.10 &73.57 &84.08 & 61.40 & 64.66  & 69.85  & 74.89  & 64.05  &89.28 &63.86 &78.72 &74.24 &81.06 \\ 
        
        ~ & \textsc{NPOS}  &96.75 &13.28 &97.22 &97.04 &97.25 & \textbf{84.76}  & 38.58  & \textbf{90.66}  & 88.32  & \textbf{91.61} &89.96 &\textbf{18.13} &94.40 &94.09 &93.56  \\ 
        
        ~ & \textsc{CIDER}  &\textbf{96.98} &\textbf{9.41} &\textcolor{blue}{97.88} &\textcolor{blue}{97.70} &\textbf{97.98} & \textcolor{blue}{84.87} & 35.97  & \textcolor{blue}{91.57}  & \textbf{89.13}  & \textcolor{blue}{92.06}  &\textbf{90.13} &\textcolor{red}{15.97} &95.09 &\textcolor{blue}{95.29} &93.92 \\
        \cdashline{2-2}\cdashline{3-7}\cdashline{8-12}\cdashline{13-17}

        ~ & \textsc{OE}  & 95.70&11.37 &97.61 &97.33 &97.75 & 74.97 & 45.83 & 87.78 & 83.97 & 89.86  &89.48 &19.70 &\textbf{95.14} &95.25 &\textbf{94.76} \\
        
        ~ & \textsc{MIXOE} &96.47 &12.30 &97.43 &97.14 &97.61 & 77.84 & 56.39 & 85.53 & 81.52 & 87.28  &\textcolor{blue}{90.49} &20.18 &94.90 &94.93 &94.37 \\ 
       
        ~ & \textsc{ATOM} & \textcolor{red}{98.03} &12.01 &96.54 &94.66 &97.45  & 83.10 &\textbf{26.31} &90.38 &87.92  &91.27 &89.61 &27.52 &89.61 &86.70 &91.34  \\
        ~ & \textsc{POEM} &95.42  &\textcolor{blue}{9.16} & 97.12 &96.21 &\textcolor{blue}{98.10}  &78.91 &\textcolor{blue}{24.49} & 89.98 &88.65 &91.39 &88.60 &29.41 &89.99 &87.65 &91.83   \\
        ~ & \textsc{DivOE} &96.68 &12.48 &96.48 &95.30 &96.76 &75.23 &27.63 &89.88 &86.99 &90.81 &89.85 &39.99 &83.54 &79.94 &85.69  \\
        \cdashline{2-2}\cdashline{3-7}\cdashline{8-12}\cdashline{13-17}
        
        ~ &\textbf{Ours}  &\textcolor{blue}{97.31}&\textcolor{red}{0.12} &\textcolor{red}{99.98} &\textcolor{red}{99.97} &\textcolor{red}{99.97} & \textcolor{red}{86.72}& \textcolor{red}{22.30} & \textcolor{red}{94.45} & \textcolor{red}{94.18} & \textcolor{red}{94.28} &\textcolor{red}{92.04} &\textcolor{blue}{17.16} &\textcolor{red}{95.63} &\textcolor{red}{95.63} &\textcolor{red}{95.03} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}
%
% Table \ref{CV experiments} shows the ID classification accuracy and the average performance of OOD detection on three OOD datasets illustrated in Table \ref{datasets}. For details of OOD detection on individual OOD datasets, please refer to Tables \ref{CIFAR-10}, \ref{CIFAR-100} and \ref{IMAGENET-200} in Appendix \ref{Experiments and visualization}. 
% On NLP tasks, Tables \ref{Llama} and \ref{text} in Appendix  \ref{Experiments and visualization} explore the performance of \textsc{GROD} using different transformer architectures and types of outliers, showing the adaptability of our method. In Table~\ref{Llama} and \ref{text}(b) with decoder-only backbones, notations ``-C" and ``-L" represent classifying with or without CLS tokens for those OOD detection methods using \textsc{Logits} only.
% For both image and text dataset formats, \textsc{GROD} consistently enhances ID classification and significantly improves OOD detection performance. Other detailed experimental results and analyses, including computational cost, ablation studies, and visualizations, are provided in Appendix \ref{Experiments and visualization}.

% \vskip -0.5cm
% \begin{table}[!ht]
%     \centering    
%     \caption{Quantitative comparison of NLP tasks, where the pre-trained Llama-3.1-8B are employed and fine-tuned with LoRA \citep{hu2021lora}.
%     }
%     \label{Llama}
%     % \begin{minipage}{0.49\textwidth}
%     \renewcommand{\arraystretch}{1.1}
%     \resizebox{0.5\textwidth}{!}{
%     \begin{tabular}{m{1.8cm}cm{1cm}m{0.5cm}m{0.5cm}m{0.5cm}m{0.5cm}m{1cm}m{0.5cm}m{0.5cm}m{0.5cm}m{0.5cm}}
%     % \multicolumn{11}{c}{~} \\
%     % \multicolumn{11}{c}{\textcolor{blue}{(b) GPT-2}} \\
%     \specialrule{0.1em}{0em}{0em}
%         \multicolumn{2}{c}{OOD Detection Type}  &  \multicolumn{5}{c}{Background Shift}  & \multicolumn{5}{c}{Semantic Shift} \\ 
%         \multicolumn{2}{c}{ID Datasets} & \multicolumn{5}{c}{\textbf{IMDB}} & \multicolumn{5}{c}{\textbf{CLINC150} with Intents}  \\ 
%         \multicolumn{2}{c}{OOD Datasets} & \multicolumn{5}{c}{\textbf{Yelp}} &  \multicolumn{5}{c}{\textbf{CLINC150} with Unknown Intents} \\ 
%         \cmidrule(r){1-2}\cmidrule(r){3-7}\cmidrule(r){8-12}
%         \multicolumn{2}{c}{Evaluate Metrics (\%)} &ID ACC$\uparrow$  &F $\downarrow$ &A $\uparrow$ &I$\uparrow$ &O$\uparrow$ &ID ACC$\uparrow$  &F $\downarrow$ &A $\uparrow$ &I$\uparrow$ &O$\uparrow$ \\ \cmidrule(r){1-2}\cmidrule(r){3-7}\cmidrule(r){8-12}
%         Baseline-L & \textsc{MSP}-L &67.67 &96.90 &\textbf{46.21} &36.04 &58.82 & \textcolor{blue}{96.00}& 31.76& 91.13& 97.50& 70.00\\ 
%         Baseline-C & \textsc{MSP}-C &53.95 &\textbf{96.03} &41.10 &35.12 &53.90 &95.89 & 26.96& 92.73& 98.11& 74.86\\ \cdashline{1-12}
%         \multirow{4}{*}{PostProcess} & \textsc{VIM} &53.95 &99.76 &40.33 &\textbf{38.00} &51.14 &95.89 &\textcolor{blue}{25.24} &\textbf{93.59} &\textcolor{blue}{98.34} &76.09 \\ 
%         ~ & \textsc{GEN-L} &67.67 &96.90 &\textbf{46.21} &36.04 &\textbf{58.84} &\textcolor{blue}{96.00} &28.84 &93.18 &97.93 &\textcolor{red}{79.35} \\ 
%         ~ & \textsc{GEN-C} &53.95 &96.84 &40.97& 33.49 &55.28 &95.89 &\textbf{25.64} &93.30 &98.24 &75.78 \\ 
%         ~ & \textsc{ASH} &64.43 &\textcolor{blue}{93.96} &\textcolor{blue}{57.66} &\textcolor{blue}{44.90} &\textcolor{blue}{65.86} &95.89 &27.16 &\textcolor{red}{93.69} &\textbf{98.30} &\textcolor{blue}{77.65} \\ \cmidrule(r){1-2}\cmidrule(r){3-7}\cmidrule(r){8-12}
%         \multirow{3}{*}{\makecell{Finetuning+ \\ PostProcess}} & \textsc{NPOS} &\textcolor{blue}{71.61} &99.99 &25.57 &27.28 &46.63 & \textcolor{red}{96.58}&43.80 &90.84 &97.60 &69.86 \\ 
%         ~ & \textsc{CIDER} &\textcolor{red}{76.26} &99.98 &24.77 &27.33 &46.14 &95.71 &37.87 &92.00 &97.87 &75.99 \\ \cdashline{2-12}
%         ~ & \textbf{Ours} &\textbf{71.15} &\textcolor{red}{83.28} &\textcolor{red}{67.00} &\textcolor{red}{57.70}&\textcolor{red}{72.42} & \textbf{95.91}&\textcolor{red}{21.60} &\textcolor{blue}{93.64} &\textcolor{red}{98.55} & \textbf{76.19}  \\ 
%         \specialrule{0.1em}{0em}{0em}
%     \end{tabular}
%     }
%     % \end{minipage}
% \end{table}
\vskip -0.2cm
\begin{table*}[!ht]
    \centering % 使内容在 wraptable 分配的宽度内居中
    \small
    \caption{Quantitative comparison of NLP tasks, where the pre-trained Llama-3.1-8B are employed and fine-tuned with LoRA \citep{hu2021lora}.}
    \label{Llama} % 建议为环绕表格使用新的标签
    \resizebox{\linewidth}{!}{ % 将表格缩放到 wraptable 环境的宽度 (\linewidth)
        \begin{tabular}{cccccccccccc}
        \specialrule{0.1em}{0em}{0em}
            \multicolumn{2}{c}{OOD Detection Type}  &   \multicolumn{5}{c}{Background Shift}  & \multicolumn{5}{c}{Semantic Shift} \\ 
            \multicolumn{2}{c}{ID Datasets} & \multicolumn{5}{c}{\textbf{IMDB}} & \multicolumn{5}{c}{\textbf{CLINC150} with Intents}  \\ 
            \multicolumn{2}{c}{OOD Datasets} & \multicolumn{5}{c}{\textbf{Yelp}} &    \multicolumn{5}{c}{\textbf{CLINC150} with Unknown Intents} \\ 
            \cmidrule(r){1-2}\cmidrule(r){3-7}\cmidrule(r){8-12}
            \multicolumn{2}{c}{Evaluate Metrics (\%)} &ID ACC$\uparrow$   &F $\downarrow$ &A $\uparrow$ &I$\uparrow$ &O$\uparrow$ &ID ACC$\uparrow$   &F $\downarrow$ &A $\uparrow$ &I$\uparrow$ &O$\uparrow$ \\ \cmidrule(r){1-2}\cmidrule(r){3-7}\cmidrule(r){8-12}
            Baseline-L & \textsc{MSP}-L &67.67 &96.90 &\textbf{46.21} &36.04 &58.82 & \textcolor{blue}{96.00}& 31.76& 91.13& 97.50& 70.00\\ 
            Baseline-C & \textsc{MSP}-C &53.95 &\textbf{96.03} &41.10 &35.12 &53.90 &95.89 & 26.96& 92.73& 98.11& 74.86\\ \cdashline{1-12}
            \multirow{4}{*}{PostProcess} & \textsc{VIM} &53.95 &99.76 &40.33 &\textbf{38.00} &51.14 &95.89 &\textcolor{blue}{25.24} &\textbf{93.59} &\textcolor{blue}{98.34} &76.09 \\ 
            ~ & \textsc{GEN-L} &67.67 &96.90 &\textbf{46.21} &36.04 &\textbf{58.84} &\textcolor{blue}{96.00} &28.84 &93.18 &97.93 &\textcolor{red}{79.35} \\ 
            ~ & \textsc{GEN-C} &53.95 &96.84 &40.97& 33.49 &55.28 &95.89 &\textbf{25.64} &93.30 &98.24 &75.78 \\ 
            ~ & \textsc{ASH} &64.43 &\textcolor{blue}{93.96} &\textcolor{blue}{57.66} &\textcolor{blue}{44.90} &\textcolor{blue}{65.86} &95.89 &27.16 &\textcolor{red}{93.69} &\textbf{98.30} &\textcolor{blue}{77.65} \\ \cmidrule(r){1-2}\cmidrule(r){3-7}\cmidrule(r){8-12}
            \multirow{3}{*}{\makecell{Finetuning+ \\ PostProcess}} & \textsc{NPOS} &\textcolor{blue}{71.61} &99.99 &25.57 &27.28 &46.63 & \textcolor{red}{96.58}&43.80 &90.84 &97.60 &69.86 \\ 
            ~ & \textsc{CIDER} &\textcolor{red}{76.26} &99.98 &24.77 &27.33 &46.14 &95.71 &37.87 &92.00 &97.87 &75.99 \\ \cdashline{2-12}
            ~ & \textbf{Ours} &\textbf{71.15} &\textcolor{red}{83.28} &\textcolor{red}{67.00} &\textcolor{red}{57.70}&\textcolor{red}{72.42} & \textbf{95.91}&\textcolor{red}{21.60} &\textcolor{blue}{93.64} &\textcolor{red}{98.55} & \textbf{76.19}   \\ 
            \specialrule{0.1em}{0em}{0em}
        \end{tabular}
    }
\end{table*}

Table~\ref{CV experiments} presents the ID classification accuracy and average OOD detection performance across three datasets from Table~\ref{datasets}. Detailed results for each individual dataset are provided in Tables~\ref{CIFAR-10}, \ref{CIFAR-100}, and \ref{IMAGENET-200} in Appendix~\ref{Experiments and visualization}. 
%
For NLP tasks, Tables~\ref{Llama} and \ref{text} (Appendix~\ref{Experiments and visualization}) evaluate \textsc{GROD} across different transformer architectures and outlier types, demonstrating its adaptability. In Table~\ref{Llama} and \ref{text}(b), ``-C" and ``-L" denote classification with or without CLS tokens for \textsc{Logits}-based OOD detection.
%
Each experiment is repeated five times using different random seeds.
%
Across image and text datasets, \textsc{GROD} consistently improves ID classification accuracy and OOD detection performance. 
%
Additional results, including computational cost, ablation studies, and visualizations, are available in Appendix~\ref{Experiments and visualization}.

